On the Robustness of Cover Version Identification Models: A Study Using Cover Versions from YouTube

Recent advances in cover song identification have shown great success. However, models are usually tested on a fixed set of datasets which are relying on the online cover song database SecondHandSongs. It is unclear how well models perform on cover songs on online video platforms, which might exhibit alterations that are not expected. In this paper, we annotate a subset of songs from YouTube sampled by a multi-modal uncertainty sampling approach and evaluate state-of-the-art models. We find that existing models achieve significantly lower ranking performance on our dataset compared to a community dataset. We additionally measure the performance of different types of versions (e.g., instrumental versions) and find several types that are particularly hard to rank. Lastly, we provide a taxonomy of alterations in cover versions on the web.

==> images/gantt.tex <==
\usetikzlibrary{patterns, arrows.meta}

\begin{tikzpicture}[
    yscale=0.8,
    xscale=1.5,
    task/.style = {draw, thick, fill=blue!20, minimum height=0.8cm, text width=3cm, align=center},
    timeline/.style = {thick, -{Stealth}}
]

% Timeline axis
\draw[timeline] (0,0) -- (10,0) node[below right] {\small Time};

% Time markers
\foreach \x/\label in {0/{Start}, 2/{Candidate Retrieval}, 4/{Uncertainty Sampling}, 6/{Worker Annotations}, 8/{Expert Annotations}, 10/{End}} {
    \draw (\x,0) -- (\x,-0.3) node[below] {\small \label};
}

% Task bars
\draw[task] (0,1) rectangle (2,1.8) node[midway] {Candidate Retrieval};
\draw[task] (2,1) rectangle (4,1.8) node[midway] {Uncertainty Sampling};
\draw[task] (4,1) rectangle (6,1.8) node[midway] {Worker Annotations};
\draw[task] (6,1) rectangle (8,1.8) node[midway] {Expert Annotations};
\draw[task] (8,1) rectangle (10,1.8) node[midway] {SHS-YT};

\end{tikzpicture}


==> images/process_fig.tex <==
\usetikzlibrary{arrows.meta, chains, positioning, shapes.geometric}

\begin{tikzpicture}[
    node distance = 7mm and 5mm, % Adjust node distances here
    start chain = going right,
    disc/.style = {
        shape=cylinder, draw, shape aspect=0.05,
        shape border rotate=90,
        text width=20mm, % Adjust text width here
        align=center, font=\footnotesize\linespread{0.8}\selectfont % Smaller font size
    },
    mdl/.style = {
        shape=ellipse, aspect=2.2, draw
    },
    alg/.style = {
        draw, align=center, font=\footnotesize\linespread{0.8}\selectfont % Smaller font size
    }
]
\begin{scope}[every node/.append style={on chain, join=by -Stealth}]
\node (n1) [disc] {\shsseed \\ 2,397 versions};
\node (n2) [alg]  {Candidate\\ Retrieval};
\node (n3) [disc] {\ytcrawl \\ 94,358 candidates};
\node (n4) [alg]  {Uncertainty\\ Sampling};
\node (n5) [disc] {\shsyt \\ 900 versions};
\end{scope}
\end{tikzpicture}


==> images/process_fig2.tex <==
\usetikzlibrary{arrows.meta, chains, positioning, shapes.geometric}

\begin{tikzpicture}[
    node distance = 7mm and 5mm, % Adjust node distances here
    start chain = going right,
    disc/.style = {
        shape=cylinder, draw, shape aspect=0.05,
        shape border rotate=90,
        text width=20mm, % Adjust text width here
        align=center, font=\footnotesize\linespread{0.8}\selectfont % Smaller font size
    },
    mdl/.style = {
        shape=ellipse, aspect=2.2, draw
    },
    alg/.style = {
        draw, align=center, font=\footnotesize\linespread{0.8}\selectfont % Smaller font size
    },
    timeline/.style = {
        thick, -{Stealth}
    }
]
% Main process chain
\begin{scope}[every node/.append style={on chain, join=by -Stealth}]
\node (n1) [disc] {\shsseed \\ 2,397 versions};
\node (n2) [alg]  {Candidate\\ Retrieval};
\node (n3) [disc] {\ytcrawl \\ 94,358 candidates};
\node (n4) [alg]  {Uncertainty\\ Sampling};
\node (n5) [disc] {900 versions};
\node (n6) [alg]  {Worker\\ Annotations};
\node (n7) [alg]  {Expert\\ Annotations};
\node (n8) [disc] {\shsyt};
\end{scope}

% Timeline below the process
\draw[timeline] ([yshift=-1cm]n1.south) -- ([yshift=-1cm]n8.south)
    node[pos=0, below] {\small Start}
    node[pos=0.25, below] {\small Retrieval}
    node[pos=0.5, below] {\small Sampling}
    node[pos=0.75, below] {\small Annotation}
    node[pos=1, below] {\small End};

\end{tikzpicture}


==> images/timeline.tex <==
\begin{center}
\begin{tikzpicture}

% Draw horizontal line for the timeline
\draw[thick] (0,0) -- (12,0);

% Draw vertical lines for events
\foreach \x in {2, 6, 10}
    \draw[thick] (\x cm,0.3) -- (\x cm,-0.3);

% Add event labels
\draw (2,0) node[below=3pt] {1 Month} node[above=3pt] {Retrieval \& Sampling};
\draw (6,0) node[below=3pt] {2 Months} node[above=3pt] {Crowdsourcing};
\draw (10,0) node[below=3pt] {2 Weeks} node[above=3pt] {Expert Annotations};

\end{tikzpicture}
\end{center}


==> images/verticalflow.tex <==
\usetikzlibrary{shapes.geometric, positioning, 3d}

\begin{tikzpicture}[node distance=1cm, auto, font=\small]

% Nodes
\node (input) [draw, cylinder, minimum height=1cm, minimum width=2cm, shape border rotate=90, align=center, text height=1.5ex, text depth=.25ex] {InputData};
\node (step1) [draw, rectangle, minimum width=2cm, minimum height=0.8cm, right=of input, align=center] {Step1};
\node (data1) [draw, cylinder, minimum height=1cm, minimum width=2cm, shape border rotate=90, right=of step1, align=center] {Data1};
\node (step2) [draw, rectangle, minimum width=2cm, minimum height=0.8cm, right=of data1, align=center] {Step2};
\node (data2) [draw, cylinder, minimum height=1cm, minimum width=2cm, shape border rotate=90, right=of step2, align=center] {Data2};
\node (step3) [draw, rectangle, minimum width=2cm, minimum height=0.8cm, below=of data2, align=center] {Step3};
\node (step4) [draw, rectangle, minimum width=2cm, minimum height=0.8cm, left=of step3, align=center] {Step4};
\node (datafinal) [draw, rectangle, minimum width=2.5cm, minimum height=1cm, left=of step4, align=center] {DataFinal};

% Time estimates
\node at (step1.south) [below=0.3cm] {Time1};
\node at (step2.south) [below=0.3cm] {Time2};
\node at (step3.south) [below=0.3cm] {Time3};
\node at (step4.south) [below=0.3cm] {Time4};

% Arrows
\draw[->] (input) -- (step1);
\draw[->] (step1) -- (data1);
\draw[->] (data1) -- (step2);
\draw[->] (step2) -- (data2);
\draw[->] (data2) -- (step3);
\draw[->] (step3) -- (step4);
\draw[->] (step4) -- (datafinal);

\end{tikzpicture}
